Scout: Rapid Exploration of Interface Layout Alternatives through High-Level Design Constraints

Although exploring alternatives is fundamental to creating better interface designs, current processes for creating alternatives are generally manual, limiting the alternatives a designer can explore. We present Scout, a system that helps designers rapidly explore alternatives through mixed-initiative interaction with high-level constraints and design feedback. Prior constraint-based layout systems use low-level spatial constraints and generally produce a single design. Tosupport designer exploration of alternatives, Scout introduces high-level constraints based on design concepts (e.g.,~semantic structure, emphasis, order) and formalizes them into low-level spatial constraints that a solver uses to generate potential layouts. In an evaluation with 18 interface designers, we found that Scout: (1) helps designers create more spatially diverse layouts with similar quality to those created with a baseline tool and (2) can help designers avoid a linear design process and quickly ideate layouts they do not believe they would have thought of on their own.

==> 9_supplementary_materials.tex <==
\clearpage
\section{Supplementary Materials}
\subsection{Spatial Diversity Score}
Here we include the formalized equation for the spatial diversity score we used for our evaluation. We compute a spatial diversity score for a pair of designs by computing for each pair of matching elements (1) the difference in position (i.e., x,y - diagonal), (2) the difference in area (i.e., $width * height$), and (3) relative distance change between any pair of elements. 

First, the \emph{position difference score} $s_\mathit{dist}$ computes the average position change between the centers for each matching element in the two layouts. Given two layouts $L$ and $L'$ with elements $L=\{e_1,\dots,e_n\}$ and $L'=\{e'_1,\dots,e'_n\}$, Scout calculates $s_\mathit{dist}$ as follows:
    $$s_\mathit{dist}(L, L')=\frac{1}{n}\cdot\sum_{i=1}^n\sqrt{(e.x-e'.x)^2 + (e.y-e'.y)^2}$$
% Discuss normalization later 
% where the scoring function measures the normalized absolute distance between the centers of the the two element.
    %The normalization constant $\sqrt{W^2 + H^2}$ is the diagonal length of the canvas (with width $W$ and height $H$), which ensures that the score to be in range $[0,1)$.
Second, we compute a \emph{size change score} $s_\mathit{size}$ to measure the average change in size for each matching pair of elements in the two layouts. Given two layouts $L=\{e_1,\dots,e_n\}$ and $L'=\{e'_1,\dots,e'_n\}$, Scout calculates $s_\mathit{size}$ as follows:
    $$s_\mathit{size}(L, L')=\frac{1}{n}\cdot\sum_{i=1}^n |e_i.width \cdot e_i.height - e_i'.width\cdot e_i'.height|$$
    % where $e.h$ and $e.w$ refers to heights and width of each elements.
    %and the normalizing constant $W\cdot H$ is the size of the canvas.
    
Third, we compute a \emph{relational distance score} score to measure how much each element moved in relation to all other elements in the layout.  Given two layouts  $L=\{e_1,\dots,e_n\}$ and $L'=\{e'_1,\dots,e'_n\}$, we calculate the relational distance score $s_\mathit{rel}$ as follows:
    $$s_\mathit{rel}(L, L')=\frac{2}{n(n-1)}\cdot\sum_{1\le i< j\le n}|\mathit{dist}(e_i,e_j)-\mathit{dist}(e_i',e_j')|$$
    where $\mathit{dist}(e_i,e_j)=\sqrt{(e_i.x-e_j.x)^2 + (e_i.y-e_j.y)^2}$ calculates the distance between centers of the two elements.  
    
Finally, we compute a spatial diversity score $s_\mathit{diversity}$ as the weighted sum of the three metrics $s_\mathit{dist}, s_\mathit{size}, s_\mathit{rel}$:
$$s_\mathit{diversity}=w_\mathit{dist}\cdot s_\mathit{dist} + w_\mathit{size}\cdot s_\mathit{size} + w_\mathit{rel}\cdot s_\mathit{rel}$$

To ensure each metric is weighted equally, we normalize the metrics into the range $[0,1]$. Given the entire set of layouts designers created in our evaluation $\{L_1,\dots L_n\}$, we compute the weights
$w_\mathit{dist}=\frac{1}{\mathit{max\_dist\_change}}$, $w_\mathit{size}=\frac{1}{\mathit{max\_size\_change}}$, $w_\mathit{rel}=\frac{1}{\mathit{max\_rel\_dist\_change}}$. 
where each weight ($w_\mathit{dist}$, $w_\mathit{size}$, $w_\mathit{rel}$ is the maximum distance, size, and relational distance change for any pair of elements in the evaluation set $L_i,L_j$, respectively. 



% -- TODO: Decide if constraint equation needed. 
% Ordering 
% \begin{equation}
% \label{equation6}
%     \begin{multlined}
%         \phi_{baseline\_grid} := \forall_{i=1}^{E}e_{i}.x == e_{i}.y \bmod c.b\_grid == 0 \\
%         \shoveleft[3cm]{\&\: e_{i}.height \bmod c.b\_grid == 0} \\
%     \end{multlined}
% \end{equation}
% \vspace{-1em}

==> ToDo.tex <==
- Amanda
    - Read through diversity and clean up motivation. Go through Chenglongs changes and see what needs to be updated
    - Architecture - cost model & equations throughout 
    - Draft quality section
    - Discussion & Conclusion 

==> equations.tex <==
    % where
    % \[
    % \begin{array}{ll}
    % G.\mathit{avg\_margin_h}=\frac{1}{|G|}\sum_{e\in G}e.\mathit{margin\_h}\\
    % G.\mathit{max\_margin_h}=\max_{e\in G}e.\mathit{margin\_h}\\
    % G.\mathit{avg\_margin_v}=\frac{1}{|G|}\sum_{e\in G}e.\mathit{margin\_v}\\
    % G.\mathit{max\_margin_v}=\max_{e\in G}e.\mathit{margin\_v}
    % \end{array}
    % \]
    % The value $e.\mathit{margin_h}$ is the horizontal margin for each element, calculated as the average left and right margin for each element in $G$ and $G.\mathit{max\_margin_h}$ is the largest horizontal margin of the elements in $G$. Element vertical margin $e.\mathit{margin_v}$ and largest vertical margin of the elements $G.\mathit{max\_margin_v}$ are similarly calculated using top/bottom margins of the elements in $G$.
    
    
    % \subsubsection{Top-level Score} 
% No need to repeat these, incorporating this into the above
% Besides assigning a score for each group in the layout idea, Scout calculates a top-level visual score to measure overall quality of the layout by treating each group as a whole.
% $$\mathit{score}_T(L)=s_\mathit{balance}(L) +s_\mathit{align}(L) $$
% where
% $$s_\mathit{balance}(L)= \frac{1}{2}(\frac{L.\mathit{avg\_margin_h}}{L.\mathit{max\_margin_h}} + \frac{L.\mathit{avg\_margin_v}}{L.\mathit{max\_margin_v}})$$
% $$s_\mathit{align}(L)=\frac{1}{|N(L)|}\sum_{(G_1,G_2)\in N(L)}\frac{\mathit{\#Alignment}(G_1,G_2)}{\mathit{\#PossibleAlignment}(G_1,G_2)}$$

% Note that the top-level scoring function reuses the group scoring function $s_\mathit{balance}$ and $s_\mathit{align}$. Scout treats each group as an element and uses properties of each group to calculate the score.

==> evaluation_brainstorming.tex <==
\begin{outline}
\1 Qualitative feedback questions (**Probably won't include the entire  list of questions in the text, but leaving them in here for now to get feedback on what might be missing**). 
   \2 What do you like about creating the wireframes in Figma? (open ended), compared to Scout?
   \2 What do you dislike about creating the wireframes in Figma (open ended), compared to Scout?
   \2 What do you like about creating the wireframes in Scout (open ended), compared to Figma?
   \2 What do you dislike about creating the wireframes in Scout (open ended), compared to Figma?
   
   
   \2 How do you think Scout would change your design process of exploring alternatives? 
   \2 What do you like and dislike about the designs you created in Scout? (specific to the designs and not the process of creating them)
   \2 What do you like and dislike about the designs you created using Figma? (specific to the designs and not the process)
   \2 How satisfied are you overall with your designs created in Scout, and Figma (overall satisfaction ranking number)
   \2 Do you have any other feedback? (open-ended) 
\end{outline}

% Conditions based on 16 participants
% 16 participants
% 8 experts 
% 8 novices 
% 4E - Social Media Scout, Weather baseline 
% 4E - Weather Scout, Social Media baseline 
% 4N - Social Media Scout, Weather baseline 
% 4N - Weather Scout, Social Media baseline 

% Each of these groups needs to have a ranking for quality 
% 24 Expert Social Media (Scout and baseline) 
% 24 Novice Social Media (Scout and baseline)
% 24 Expert Weather (Scout and baseline) 
% 24 Novice Weather (Scout and baseline) 


% Notes from James: 
% Usage logging
% Expertise
% How many did they explore? 
% How satisfied are you with the designs? Is there a scale? This can be quantifcation 
% Diversity and quality 
% IdeaHound -look to it for measuring diversity
% Ranking quality % 
% Equivalence buckets 
% Articulate why they ranked them that way 
% What is it about the designs that 
% novices rated higher if made by scout 

% Feedback qualitative 
% Constraint certain values 
% Plot time  -- patterns of feedback
% Paper - wireframe -- look 
% Remove the constraints all at once & start from scratch 

% Organized 
% - Clear groupings of elements - Can understand what belongs together
% - Main point of emphasis 

%  Defining Organized
%   - Clear grouping of elements - 
%   - Alignments
%   - Symmetry - 
%   Defining energetic
%   - Has one main point of emphasis - How would we measure this? 

% Measures of simliarity have been introduced - minukovich et al compute image features visual similarity - however, majority of features are color based and not capturre granular enough values. Additionally, spaital similairty metric does not capture high magnitudde of difference due to large amount of white space in our designs. Heil, et. al. introduce simliarilty meausre based on Gajos simliiarty measure where each widget is compared along a lineaar combination of features (eg.., ). in our case, we have this set of factors (position, size, neighboring elements, representation) to capture dissimliarity of two wireframes. Also cpature information about difficult of transforming interface from one representation to another  - normalilze by distance on teh screen, 
% Weights - how would we get the weights for the model? - need to have reasoning for initial set of weights - 0.25 each (?) https://www.sciencedirect.com/science/article/pii/S0010027702001841
% Similarity as transformation

% With our metric - since we know the corresponding matching lement - aim to capture also amount of effort rqeuired to transform the design - along w/ spatial metric 
    
% For diversity, we would compute the average difference score from the pairwise comparison for each design within a single designer's designs, and then report the results for each condition. 

Ways of measuring diversity/similarity of designs
- Visual image descriptors. \cite{miniukovich} - Challenges: Many metrics focused on color, not relevant for our task. Doesn't capture change to individual component - components are not linked to each other. 
- Document layout similiarity - based on overlap - not linking components



% Describe diversity metric 
% Justification & Figure showing designs side by side.

% Diversity metric 
% Visual Diversity and User Interface Quality 
    % Minukoviuch metrics - Image Descriptors --mostly about color, enough difference to distinguish as using same components, and no colors 
    % Also could use MPEG-7 structural simialrity index - but this doesn't seem to produce enough difference for black and white wireframe, given that most of deisgns is whitespace. 
    % http://www.keysers.net/daniel/files/Beusekom--Layout-Distance--DIAL2006.pdf
    % Proposed layout measure for document similarity - Some methods depend on overlapping components - our components may not neccessarily overlap - Document Image Retrieval Based on Layout Structural Similarity
    % 
    % For alternate representation - Gajos paper - can be another dimesion 
    % Spatial pyramid matching -  
    
    % Layout based web similarity feature - % https://www.sciencedirect.com/science/article/pii/S1071581917301465
    % https://link.springer.com/chapter/10.1007/978-3-319-48740-3_18 - 
    % CBR - AI based - 
    
    % QUALITY EVALUATION
% For quality, the overall results were (TBD). 
% - Quality - how well the designer is able to achieve their design goal
%     - Clean - Well aligned, balanced
%     - Compelling - Has a clear main focal point. - Measure with saliency model. 
%     - TODO: % Invesigate whether saliency model will work for measuring. 
%         - Measuring point of emphasis - Get saliency model & patches, threshold the image above a certain value of saliency
%         - Find connected components
%         - Is there a largest component and how much larger is it - take into account the saliency values
%     - Measuring alignment, clutter
%         - Use alignment from cost function
%         - Use clutter metric
%         - Compute symmetry on designs
%     - alignment (number of total alignments), balance/margin (padding in groups consistent), size (within a group), 
    
    
    % Potential arguments for a more automated approach 
% clean, uncluttered as attributes 
% Defined as well-aligned, balanced, and uncluttered 
% Can use cost function to evaluate a score 
% Compare the baseline designs to the Scout created designs
% Alignment, balance are well known quality metrics of a good layout (several sources), and uncluttered as welll (cite), so these are good measures independently. Some papers have automatically measured these (odonovan, mobile layouts one) attributes
% -- alignment metric uses groupings - how would we measure if we don't know the groupins for the baseline design? Scout will encourage grouping elements, but baseline won't necessarily 
% -- clutter metric only uses element size so should be possible to evaluate. 
% Is this biased towards Scout? - The designer is not required to choose the designs ranked first in the list of ideas. 


% Rough interview outline 
% After baseline task 
%   - Describe the process you followed when thinking of and creating the alternative wireframe layouts in Figma 
%   - What process would you follow, more generally (in a typical context), and how does that differ for this task? 
% After Scout task 
%    - Describe the process you followed when using Scout to explore alternative wireframe layouts? 
% After both tasks
%       - Thinking back to the process you followed in both, how do you think Scout might change this process? (Reflect on the differences between the two processes) 

% Other interesting possible questions/data
% - What is the potential impact on diversity/brainstorming process & helping them think of new ideas? How do designers think Scout could impact the diversity of their designs?  

% - What is the impact of design expertise on the above? How does the process differ with those w/ high design expertise vs low? What is the impact on the resulting layout ideas? 

% - What is the impact on diversity of the design they produced if they complete Scout task first, and then do the baseline task? For RQ1 above, we could look at how the diversity score is impacted by the ordering in which the tasks are done. Also look at diversity across the full set of designs, and contrast to within a single designer diversity 

% - What other aspects of exploring diversity are we missing? Is there something that Scout might be missing to help it make designers explorations more diverse? (not sure how to ask this, but in general, it would be nice to get their thoughts on aspects of variations that the designers would like Scout to explore, or other types of feedback they might want to give, but feel like Scout might be missing) 

% Other concrete things we could look at
    % - How much sketching did they do in both conditions? (Did they sketch at all? How much time approximately did they spend sketching vs in Figma) 
    % - In Scout, report how many designs they saved and discarded. This can provide a contrast w/ baseline condition where they explored ideas in their head or on paper but we can't capture how many ideas they explored in their head
    % - In Scout, report how much feedback, types of feedback the designers used, how much (not sure if this will be interesting?)  

% Results
% What were the processes followed by designers in the baseline condition? What were the processes followed by the designers using Scout? What are the categories of reflections they made? What were the interesting differences that they pointed out? 


% - Evaluation 
%     - Depends on quality or quantity 
%     - What is the prompt? 
%         - Context
%         - Diversity or just create the best design possible
%         - Trained designers typically want to create diverse alternatives
%         - #2 - How to measure it? Would an expert measure diversity? 
%         - Counting - How do we count how many designs they explored? 
%         - What is a measurement that makes them comparble? 
%         - Prompt: Pick your favorite designs. 

==> leftovers.tex <==
Additionally, more designers thought that their \hl{(1) Scout designs were more "compelling".} However, "compelling" to them did now always mean having a clear point of entry and a clean hierarchy, but could instead mean "different", "interesting", or "atypical". 


% P4 
% Compelling - It does a good job w/ the compelling thing
% The hiearchy is not dull or boring 
% Its not really even familiar 
P4 -- It does a good job with the compelling thing, it definitely like the hierarchy is not dull or boring or and to some extent is not even familiar <laughs> cause it does break, like for example this one does break ... like this one <points to one Scout design>, it breaks cliches that's for sure. Like it does a good job of not being boring but clean I wouldn't say that.


While Scout showed potential in our evaluation for avoiding design fixation, \hl{(2) the designers felt that the designs they created without Scout were more \textit{clean}} when explicitly comparing the two sets of designs (10 designers without Scout vs. 5 with Scout).



% P10 
% I guess ii terms of cleaner and compelling - XD helps more - in my thinking Scout can give you diverse layouts - rather than clean - sometimes the sizing in Scout or proportions of components - you need to fix that afterwards - at least for me I had to change some size and position issues in the Scout ones. 
% I think still manually people - or designers - would still need to fine tune and make changes to it.
P10 --

% P17 
% Think they are compelling but maybe not as clean 
% b/c i had to do some work to clean them up 
% Just given from Scout - there wasn’t really proper alignment of things - and then sizing and consistency was a bit off - That was what the most spent time on 
% Cleaning and organizing it
% Not as strong in this task - but i do think they are compelling
P17 -- 


% P20 
% Think clean is hard b/c you’d have to put a lot rules to get it as clean as you might want it to be 
% This one (right one) not very clean looking but i could picture moving around where it would be clean 
% Definite on diversity it gave me a lot 0- seemed more effort in Scout to make it clean than it would in XD 
% Compelling - hard to see when its not clean 
P20 -- I think clean is hard because you'd have to put a lot of rule on it i think to get it as clean as you'd want it to be. For example this one i picked is not very clean looking but I could picture moving it around a bit and it would be clean. Definitely on diversity it gave me a lot, but clean, it seemed like more effort to make it clean in scout than it would in XD. 
R -- How about compelling
P20 -- It's hard to see when it's not clean





We can think of a few possible explanations for this. First, the amount of time that designers had for the two tasks was the same. However, Scout requires an initial process of specifying grouping, ordering, and emphasis before generating design ideas which may have left less time for cleaning up the design ideas during the refinement stage of the Scout task. Second, a few designers mentioned that they would need time to develop trust in the tool, and that they felt they needed to check the low level details of the designs (i.e., fonts, sizes) before they could trust that the designs were "clean". 

While the designers believed the designs they created with Scout were less clean, Scout expanded the designers capabilities in other ways. 


\textbf{Scout helped designers focus on structure first rather than details.}


Another key way that Scout helped designers in our study was \textcolor{red}{\hl{(3) in considering the high-level structure of a design before the low-level details.}} When asked to compare their design processes with and without Scout, more designers mentioned considering emphasis of specific elements with Scout (13 designers) than without Scout (11 designers). More designers mentioned considering the high-level grouping structure with Scout (14 designers) than without Scout (6 designers). Finally, more designers mentioned considering the order of elements with Scout (7 designers) than without Scout (1 designers). 4 designers also mentioned that Scout could provide a more structured process for their design and improve their mental model. 

% P17 
% In Scout i had more intention - behind some of the choices i made - the selections - and also the structure - got me thinking of things on my own - (also talks about avoiding bias)
P17 -- 

% P10 
% Scout can generate a bunch - however you also need some time - you have to spend time to setting it up (grouping, order, importance) - training up it -and then need to assign some attributes to the machine to let it generate for you - but i think when i used Scout - i still need to consider which elements are more important and figure out the relationships between them - It can be a good way to keep me in the right track - in terms of thinking of priority - its like creating a spec before i begin **good quote*
P10 --


\textbf{Scout helped designers resist design fixation.}


However, breaking conventions was not always seen as a design goal. \hl{(4) 2 designers mentioned that some familiarity in design is good} and that they don't like breaking design conventions too much. 

% P4 -- (not the full quote probably, but pick a good subpart)
% A weather app is universally recognizable 
% There is only so much iteration across ways to present the information 
% Trying to diversify too much it could be distracting or confusing for the users
% Personally - a design principle I subscribe to is that familiar is good b/c it makes it so people don’t have to think too much with your app or dig around to find the information
% I struggle to diversify because of that
% My creativity was also constrained (due to the rules of the task)
% Maintaining the sense of familiarity is something i priortized in my designs because I don’t see that as a negative thing
% ---
How successful do you feel you were at creating diverse designs with Adobe XD?
P4 -- As much as I wanted to diversify, in my head i had a clear heirarchy of how the information should be laid out. What infor is the most prominent. Weather apps is one of those things that is very universally recognizable. When you look at like weather reports on television right, on the weather channel, there is only so much iteration on the ways they present the information. Because if you try to break the mold, if you try to diversify too much, it only serves to be distracting or confusing for the user. Like beacuase I saw in the report one thing they mentioned, they called it [reads off flyer] familiar, looks like other web app screens. Personally like one of the big design principles that i poersonally subscribe to is that familiarity is good, in a way. Because it makes it so that people don't have to think when they're using your app. They don't have to like dig around for different sources of information or something like that. Yeah so kind of, for me, doing this excercise with this weather app where there's a very clear cut line of thinking in terms of infor heirarchy, fo me it was a bit of a struggle to diversify the different ideas just because i felt my creativity was constrainted by all these parts of the task. Infor heir and in terms of maintaining that sense of familiarity such that the app is actually navagatable. I prioritize more on usability and familiarity and less on diversity. 

% --- Another option 
% P15 
% With a weather app - instead of reinventing the wheels again - I try to play w/in the existing pattern - thinking about the important information that users are trying to get - didn’t diversify that much that ii think about it - just played with it - now that i noticed it for some of them, i used the icons - but this one is interesting - it has the Sunny - the icon can be confusing possibly - so you might want to maybe  use words that can can convey the message better - i wouldn’t say they are not very different from each other but they are different
% ---
P15 -- 


Additionally, \textcolor{red}{\hl{(5) Scout helped the designers resist design fixation and think of outside the box ideas.}} 11 designers mentioned that some or all their Scout designs were different than a typical weather or social media profile screen, which are common app types that frequently use conventional layouts.  

% P1 - Followers/Following numbers - saw them arranged the same way in other apps, so she thought thats how they should 
P1 -- 

% P7 - showing ineffective designs - stretches your understanding of whats possible, more like using an editorial skill set -- good quote 
P7 -- 


P10 --

% P10 - 2
% When there are previous existing screens like this - it can be hard to brainstorm because previous screens like that (existing) - It can make me annoyed to think of different ways to layout the components - 
P10 --

2 additional designers mentioned that \textcolor{red}{\hl{(6) Scout helped them break out of their "personal style".}} 




First, \hl{(7) Scout helped designers think of new ideas they might not have thought of on their own (9 designers).} 

 
P16 -- 

% P9 
% Scout was interesting because it did a lot more combinations of all the elements than i would have been able to think of. 
% Played with the sizing/pos in ways i wouldnt have thought of ** good quote **
% Every designer has a style 
% Scout made more layouts than the ones limited to that style the designer would have
% It made me think of other arrangements that could be used
% b/c it made them i could decide and see whether i could like them or not 
% Not sure i could have come up with them myself - 
P9 --

% P11 
% I guess that i ended up putting more effort into designs that - i am not good at using the whitespace more intentionally - i have this bad habit of forcing myself to go through multiple iterations in print design -I  refine until i have a lot of whitespace - I will end up having much more than i tend to have in the initial design - I feel like the options i chose from Scout kind of reflect my desire to be a more intentional user of whitespace
% Wouldn’t have come up wiht this L shaped whitespace (alt1) (in the Scout designs) - And the blocks of whitespace (alternative 3)
% Later on i would refine these and try out the more variations - In the initial phase i hardly ever come up with wild uses of whitespace like scout did - really appreciated that
P11 --

% P2 
% I wouldn’t have thought to put the image in the bottom of the page
% This gigantic (sunshine) one 
% Scout helped with that 
Scout post task - What strategy did you use to come up with the alternative designs?
P2 -- so i knew that i wanted to group some pieces of information and i also wanted to maintain some heir of inform. So that's why i put those rules in. so the way scout helped with that was also, i wasn't even looking to make something like the third layout. Iwouldn't have thought to put this, put the image at the bottom of the page. This gigantic one. So I think Scout helped with that. Although it did take a while to figure out what I wanted out of it. 



% P1
% Scout helped me come up w/ more diverse and intriguing alternatives. The designs felt a touch dull when creating it on my own
% They are some ideas i wouldn’t have thought of, makes for more interesting designs
% Scout helped me come up w/ more diverse and intriguing alternatives. The designs felt a touch dull when creating it on my own
% They are some ideas i wouldn’t have thought of, makes for more interesting designs
P1 --



\textbf{Designers would use Scout during concept ideation.}

X designers mentioned that \textcolor{red}{\hl{(8) Scout could speed up their current brainstorming strategies.}} Designers mentioned using a number of strategies to think of new layout ideas including sketching, whiteboarding, and looking for examples. 13 designers also mentioned using the canvas to think of ideas by placing elements and then moving them around. With Scout, designers believed they could explore many more layout ideas quickly than they could sketch by hand or visualize by moving elements around on a canvas.  
Some designers mentioned they'd like Scout to hook into design asset libraries or have an option to conform to their org's design guidelines. 

% P18 
% Scout would be useful to just generate a bunch of ideas really quickly 
% And for testing things out really quickly - in terms of alternative shapes - i really like that part of the tool 
P18 --

% P11 -- love this one 
% Sketching is a high effort activity 
% I don’t just output the ideas that come across my mind
% When i sketch i am preselecting them b/c i twould take me time to concretize them on the paper 
% So there’s def a ccost benefit evaluation - Scout - somehow bypasses - helps to mitigate that - it has some wilder ideas - some of mine (with the weather app) seem like they wouldn’t come from Scout - which is fine  bc i can always change in XD later on - but i guess that the value for me was in the first workflow - was to visualize a much bigger array of variations that i would have otherwise
P11 -- 

Finally, we wanted to understand how and whether designers could see a tool like Scout fitting in to their design process. 14 designers said that \hl{(9) they would use Scout as an ideation tool, or to quickly visualize many design possibilities.} 

% P13
% w/ Scout - it kind of already gave me the layout - choose the one i like - make small changes later - a cleaner workflow - then i don’t have to create so many artboards and then moving a lot of things around 
P13 -- 

% P15 
% Sticking w/ just XD - would say its’ not a fair comparison b/c i would use dribble (or other searching for ideas) - Scout can generate them instead - you can see a lot you didn’t think of - Scout would be doing a good job - on dribble - its a sea of information need to narrow down - with Scout - you give it the logic and then it comes up with the information (so there might be less things to narrow down since you’re already working with your own information)
P15 -- 


% P5 
% Was definitely kind of a more time consuming b/c i wanted to see things up front to see if certain concepts would be worth creating. 
% For the last one, i put the profile picture on there right w/ the name and title next to it, took a while to kind of get there and remember playing around w/ the information right next to the profile picture but would have been nice to quickly see that i didn’t want to put everything up there. 
How did your approach to creating alternatives using Scout and Adobe XD together differ from your approach using Adobe XD alone?
P5 -- XD alone it defiinitely felt like all the emphasis wa on me to kind of decide how things, where... I'd say it was def kind of a ... i'm trying to think of the word... it was def more time consuming because I wanted to see a bunch of diff things upfront, just to see if different concepts would even work. Sort of the last one I did, I remember the profile picture on the right and then putting the name and title up next to it, that took a while to get there. I also rememr playing around with like putting all the information right next to the profile picture but it would have been nice to quickly see that like i didn't want everything up there, I just wanted profile picture, name and title. 


% P17 also had a good quote about brainstorming and ideation being like braiding but not sure I can make sense of it. 


% P6 
% Once you got the results, it helps , instead of searching on the internet, it makes it with the information you already have, and see what it could look like with information you have. 
Think about the last interface you created (before this study). Did you try to find alts? How could Scout help with that?
P6 -- I guess like it, for me what i foudn difficult was just setting the constraints or whatever in the beginning. But like once you got the results, definitely it helps instead of like i guess searching on the internet for alternative layouts or exisint gthings that are out there. it just kind of makes it easy with what you already have, so I guess it's easier in that sense that you already see what it could look like with the information that you have, and not other information. I guess the one thing that turned me off was setitng the constraints. But i don't know maybe that's a necessary thing. 


4 designers mentioned they would \hl{(10) use Scout when stuck and in need of inspiration,} while 6 designers noted that they struggled in thinking of ideas during the baseline task. 

% P2 
% Most likely in the initial phase when i’m first designing it 
% It could maybe replace sketching for me 
% I do see it as helping me start 
% Or if i have a time i get stuck or a creative block
How could you see yourself using a tool like Scout in that process?
P2 -- most likely in the initial phase when i'm first designing it. probably i could see scout replacing sketching for me. I see it as helping start. or if I have a creative block I need to get rid of.

% P2 - regardinig baseline task 
% Feel like i was able to create two good designs
% Wasn’t able to come up with a good third one
% I wanted more time or more time sketching 
How successful do you feel you were at creating diverse designs with Adobe XD?
P2 -- i feel ike i was able two really good designs but the middle one I really don't like. I wasn't able to come up with a third one. so i feel ike I probably just needed more time sketching it out. 

% P4 
% I struggled in the first one (Baseline task) with brainstorming and ideation. 
% This tool (Scout) made brainstorming a much easier process for me personally
How successful do you feel you were at creating diverse designs with Scout+Adobe XD together?
P4 -- If anything, it was way quicker for me to come up with these three. What I struggled with the most on the first one [the first Baseline task] was really brainstorming and ideating, these sort of different variations. Scout made brainstorming a much easier process for me personally. 


% P7 
% Using Scout - i was able to focus primarily on rearranging the possibilities created by Scout
% With XD - I had to imagine the possibilities and contest with my own self-assessment of not being able to meet the goals
% My ego got in the way - I was freed from that in Scout 
% With the baseline - I looked at this - i had no inspiration of how to make it particularly different
% Self-assessed the lack of inspiration and thought a better designer would have had more inspiriation 
% This set the tone for my work as i went through the alternatives
% Had an internal critic - this isn’t good enough but you can’t figure it out. 
% More focused on
P7 -- 

\textcolor{red}{\hl{(11) Scout also made or could make the designers' design process less linear.}} Either after completing our study task without Scout, or when thinking about a previous project, 12 designers mentioned sometimes following a linear process of looking at a design and thinking about how to change it to make a new design, while only 2 designers mentioned a linear design process in Scout. With Scout, they could instead quickly visualize a variety of spatially diverse design possibilities, and resist focusing in on a few designs too early. 

% P7  -- love this quote!
% Oh my god. 
% Like every day - would use it to come up w/ those alternatives is huge. 
% The accomplishment there is to free yourself from one linear approach. 
% Reaction style approach is just one person following a train of thought, but it would be only one path
% Using something like this - each with a team of designers - as a starting point - to be given a half dozen different thread i can follow to refine (would be useful)
P7 --




%Our interviews with designers also . surfaced a few key improvements. During the study tasks, designers struggled to understand and apply some of Scout's feedback options and constraints. Future versions of Scout could present the feedback options, and better scaffold the designers' learning process for both feedback and constraints. Additionally, Scout could support more inputs and outputs such as importing from style guides and component libraries, and allowing designers to specify ranges and specific values for feedback variables. 

%Finally, Scout could allow designers to combine sub-parts of designs. 11 designers mentioned  liking a sub-part of a Scout design, but they would want to combine it with one or more parts of other designs to create a new variation, or "mix and match" the designs.
%-- \\
%TODO: Maybe insert quote ?? \\ 

% P2 
% It was helpful 
% I feel like I created 3 very diff designs 
% Everything about the layout was different 
% I did need to further refine them
% Was able to pick up a couple of good aspects of  any given layout and then felt like i would want to mix and match


%--\\

% Diversity metric
%  For RQ1, we wanted to understand whether Scout could help designers explore more diverse layout ideas, thus we needed a robust diversity metric. Researchers have used many approaches to measure design diversity, but have not yet created a standardized metric to robustly compare two interface wireframe layouts for diversity (i.e. dissimilarity). We found that vision based approaches \cite{miniukovich2015visual} are not well-suited to comparing low-level wireframes as they are made up of a majority whitespace, and thus computing pixel differences does not provide a fine-grained diversity measure or capture the transformation effort required to convert one layout to another


% A related effort by Hahn, et. al. \cite{hahn2003similarity}, showed that the dissimilarity of two layouts is highly relates to transformation distance, or amount of changes required to adapt one representation to another.. 


% New ideas - woudn't have thought of 
% P16 
% First one is pretty similar -but it has diff font size - and locations - I wouldn’t have thought to use the larger font size with the smaller header 
% So it’s pretty fascinating 
% Would not have ever made the font so big in comparison to the photo - its a good wireframe -

% Resist fixation
% P9 --- 
% I focus on my personal style
% Scout breaks out of that by showing a broad range of ideas ** good quote **
% I could generate new ideas to have it show me more 
% Just shows me more possibility and opens my eyes to how things could be arranged that are atypical
% Often times when i design - its based on what i have seen and what i’ve liked - it (Scout) comes up with its own things 
% --- 
% P10
% For profile pages - they have a settled layout already within a bunch of apps you use - they have a similar layout in terms of followers - Scout generates diff groupings - you won’t keep all of them -  sometimes it depends on the type of screen you want to generate

==> order.tex <==
- Constraints section
- performance and scalability
- Synthesis
- related work
- intro 
- Cost function
- Evaluation
- Throw discussion bullet points in as going along through the rest. 


- Score thoughts
  
  
- Normalize by the max distance for that pair of elements or largest size change in that group we are comparing 
- 

==> study.tex <==
----- New User Study Plan ----- 
What am I evaluating? 


Research Questions 
 RQ1: Does Scout help designers create a more diverse set of interface design alternatives? 
 RQ2: Does Scout help designers create higher quality design alternatives? 
 RQ2: How does/will Scout change the design process of designers as they create design alternatives?

    
User Study Process & Workflow
- Demographic Survey - 5 minutes
- Scout Tutorial - 20 minutes
- 2 Tasks - 20 minutes each 
- Post Survey and Feedback - 15 minutes. 
- Total time - 1.5 hours. 
    
Participants
- Participants will be professional interface designers
- We will recruit them from LinkedIn contacts, through email, and through DUB mailing list and other designer facebook groups by sending out a survey link to indicate they are interested. 
- They will have 1 year minimum professional design experience 
- We will recruit 10-16 (probably an even number so that the conditions and tasks are balanced).

Study Workflow 

Pre Survey 
- Demographic data collection survey will gather demographic data and information on their level of design experience. 

Tutorial Tasks
  - Designers will complete a Scout tutorial before beginning (20 minutes)
  - This tutorial will walk them through the features of Scout and give them 1-2 practice tasks to get used to the interface. 
  - As the designers will already be experts in Sketch, we will have them learn how to use Scout first so we can have a more even baseline. 
  
Conditions
    - The study will be within subjects. Each designer will complete one task under each condition. 
    - The order the designers complete the conditions will be counter-balanced across designers
    - The study will consist of 2 conditions: 
        1) Baseline (Sketch Design Tool)
        2) Scout
Tasks
  - There will be two tasks. Each task will be limited to 20 minutes. 
  - For each task, we will give the designers a set of components to work with to create the screens. 
  - These components will be chosen to fit a particular type of screen (e.g., Social Media Profile) with a fixed set of components. 
  - The designer will be required to use a fixed set of components but not all of the components will be required and some will have alternative representations. 
  - We will ask the designer to create the 5 best alternative designs that they can within 20 minutes, and to try to make them as diverse as possible. 
  - These will NOT be think-aloud tasks as we want the designers to focus on creating high-quality designs and that could potentially be distracting. 
  
Post Survey 
  - We will give them a post Survey to compare their experiences using the two modes of creating alternatives. 
  - We will ask them for how they think Scout could change their process of creating alternatives, and to give general feedback on how we can improve Scout 

Answering RQ1 - Measuring Diversity
- There will be two metrics measured. 
    1) Computational metric where we compute the spatial (x,y,size) distance away from all other designs created from a Designer-Task-Condition combination. 
    2) Expert ranking of diversity where we ask them to compare pairwise how different each set of designs is (Or a better way) 
    
Answering RQ2 - Measuring Quality 
- We will have an expert panel rate the quality of the designs. 
- Expert panel will have 2-3 designers
- Expert panel will be recruited through UpWork and we will send them the designs to rank and a rubric. 
- The will rank the entire set of designs for a single task
- They will evaluate the designs according to an evaluation rubric (TBD) 

Answering RQ3 - Alternative Creation Impacts
- We will answer this from the qualitative feedback survey that designers will fill out (online in a form) after finishing the tasks. 
- We may also interview them with these questions to get more candid feedback. 


==> timeline.tex <==
Remaining Tasks
- Draft Quantitative results (spatial diversity score) 
- Draft Motivating Example 
- Draft Qualitative results 
- Finish Intro/Architecture details

Chenglong tasks 
- Draft diversity score description (with formula) 
- Draft cost model section

Summer Timeline 
June 9 - 15 
- Amanda - Draft motivating example - Figure of Scout interface 
- Amanda - Finish architecture (Amanda's parts) and Intro 
- Amanda - Recruiting evaluators for quality of designs

June 16 - 22nd 
- Chenglong - draft diversity score writeup 
- Amanda - Draft qualitative results section
- recruiting evaluators for quality of designs

June 23 - 29th
- Chenglong - draft cost model writeup
- Amanda - Draft quantitative results (spatial diversity scores) - getting feedback on 14th from Lisa Elkin around ART analysis - after that can draft once confirming analysis seems correct. 
- Alannah - Read/edit draft of qualitative, help find quotes 

June 30th - July 6th 
- Alannah - Read/edit draft of qualitative, help find quotes 
- Amanda has week off of 4th of July. Will work on various parts of draft 
- Send full draft to Andy/James for reading/feedback

July 7th - 13th 
- GOAL: Have full draft (possibly sans quality evaluation of designs) for reading/feedback. 

July 14th - 20th 
- Addressing feedback/comments

July 21st - 27th 
- Address feedback/comments

July 28th - Aug 3rd 
- Have quality evaluations done by evaluators at this point
- Draft quality evaluation 
- Complete draft done 

Aug 4th - Aug 10th 
- Address feedback/comments, clean up figures, etc.

Aug 11th - Aug 17th 
- Address feedback/comments, clean up figures, etc.

Aug 18th - Aug 24th 
- Address feedback/comments, clean up figures, etc.

Aug 25th - Aug 31st 
- Address feedback/comments, clean up figures, etc.

Sept 1st - Sept 7th 
- Last week at MSR

Sept 8th - Sept 14th 
- Make video 
- CHI Abstracts/Metadata due (Sept 13th)

Sept 15th - Sept 20th  
- Make video 
- CHI Submission Due (Sept 20th) 


==> timeline_2.tex <==
Timeline

March 18-22nd
- Define metrics & refine methods 
- Create Scout tutorial
- Pilot Scout tutorial
- Refine task components and fix bugs 

March 25 - 29th 
- Continue refining metrics
- Pilot tutorial
- Make last system improvements for task components
- writing

April 1st - March 5th 
- Make last system improvements for task components
- Partial piloting w/ tutorial and Scout
- writing




































April 8 - April 12th 
- Partial piloting w/ tutorial and Scout 
- writing

April 15 - April 19
- Full piloting
- writing

April 22nd - April 26 
- Recruiting and scheduling participants. 
- Full piloting
- writing

April 29th - May 4th
- Recruting & scheduling participants
- Full piloting
- writing 

CHI - Vacation

After
20th - 24th 
- Conduct study 
- Analysis
- Writing

27th - 31st 
- Conduct study
- Analysis 
- Writing

3rd - 7th 
- Analysis 
- Writing 

10 - 14th 
- Analysis
- Writing

17th - Start internship



Piloting plan & Timeline 
    
Potential Pilot Participants 
- Jasper
- Eunice 
- C&C lab 

Piloting process
 - For baseline
    - Set up a Figma document with instructions, the task, and components 
    - Send a link (with editing privileges) 
    - Ask them to create (3-5) alternative designs within 20 minutes. 
    

Tasks---- 
Recruiting Tasks: 
- Collect emails of previous designers to recruit + previously contacted. 
    - Fill out our Screening Survey (Already made) 
- Send out recruiting survey through Facebook and DUB 
- Make Doodle poll for participants who respond to fill out for scheduling 
- Scheduling participants
    - Booking a room in CSE or Gates
    - Email participants w/ a time slot

User Study Tasks
- Cleanup and normalize task components
- Cleanup/Time Scout tutorial  
- Make post survey for feedback and qualitative data. 

Statistics
- Figure out how to compare the diversity across conditions (What types of stats to use? 





    
    



